The Need for Seed (in the abstract Tile Assembly Model)

In the abstract Tile Assembly Model (aTAM) square tiles self-assemble, autonomously binding via glues on their edges, to form structures. Algorithmic aTAM systems can be designed in which the patterns of tile attachments are forced to follow the execution of targeted algorithms. Such systems have been proven to be computationally universal as well as intrinsically universal (IU), a notion borrowed and adapted from cellular automata showing that a single tile set exists which is capable of simulating all aTAM systems (FOCS 2012). The input to an algorithmic aTAM system can be provided in a variety of ways, with a common method being via the "seed" assembly, which is a pre-formed assembly from which all growth propagates. In this paper we present a series of results which investigate the the trade-offs of using seeds consisting of a single tile, versus those containing multiple tiles. We show that arbitrary systems with multi-tile seeds cannot be converted to functionally equivalent systems with single-tile seeds without using a scale factor > 1. We prove tight bounds on the scale factor required, and also present a construction which uses a large scale factor but an optimal number of unique tile types. That construction is then used to develop a construction that performs simultaneous simulation of all aTAM systems in parallel, as well as to display a connection to other tile-based self-assembly models via the notion of intrinsic universality.

==> imposs-scale1.tex <==

\subsection{Scale factor 1}


In this section, we prove that there are infinitely many aTAM systems whose seeds consist of more than one tile, but for none of them does there exist a singly-seeded aTAM system which can produce the exact same set of terminal assembly shapes, which also implies that none of them can be seed-growth-simulated by any singly-seeded aTAM system.

\begin{theorem}\label{thm:imposs-scale1}
There exists an infinite class of aTAM systems, $\mathfrak{T}$, such that for every $\mathcal{T} \in \mathfrak{T}$, there exists no singly-seeded aTAM system $\mathcal{S}$ which shape-simulates $\mathcal{T}$ at scale factor 1.
\end{theorem}

\begin{proof}
We prove Theorem~\ref{thm:imposs-scale1} by first presenting an aTAM system $\calT = (T,\sigma,1)$ and then showing why it cannot be shape-simulated by any singly-seeded aTAM system. A high-level overview of $\calT$ is shown in Figure~\ref{fig:no-single-seed-at-scale-factor-1}. The seed $\sigma$ consists of $5$ tiles (shown in grey and labeled $A$ through $E$). Growth can happen in two locations: from the north of tile $A$, and south from tile $D$. The green tile can attach to itself and grow an arbitrarily tall column of green tiles. However, nondeterministically and at any point either a red or blue tile can attach. The red tile has no glues on its north, east, or west sides, and thus terminates the growth of the column. The blue tile is among a set of tiles which are able to attach and grow four positions to the east, and then a single tile type which attaches to itself (on the north and south sides) and grows downward until it crashes into tile $E$ of the seed. Analogously, the yellow and pink portions may grow on the south.

\begin{figure}[t]
    \centering
    \subfigure{
    \includegraphics[height=50mm]{images/no-single-seed-at-scale-factor-1-2.png}
    \label{fig:no-single-seed-at-scale-factor-1}
    }
    \quad
    \subfigure{\raisebox{19mm}{
    \includegraphics[height=31mm]{images/SF1-blocking.png}}
    }
    \caption{An example system from the class $\mathfrak{T}$ which cannot be shape-simulated by any singly-seeded aTAM system at scale factor 1. The left and right show two possible terminal assemblies. The grey tiles (labeled $A-E$) are the seed. Green tiles can grow upward arbitrarily far, and at any nondeterministic location either a red tile can attach to terminate the growth of the column, or a blue tile can attach which causes growth of four additional tiles to the right and then growth downward of a column which crashes into the tile labeled $E$. Similar (but slightly narrower) growth can occur with the yellow and pink tiles, initiating from the tile labeled $D$.}
    
\end{figure}

We now prove that $\calT$ cannot be shape-simulated by any singly-seeded aTAM system by contradiction. Therefore, assume that aTAM system $\mathcal{S} = (S,\sigma',\tau)$, where $|\sigma'|=1$, shape-simulates $\calT$ at scale factor 1. We now do a case analysis to show that there is no valid location for the tile of $\sigma'$ to be placed such that $\calT$ can be correctly shape-simulated.

Each of the following cases assumes a different location for the tile of $\sigma'$ and shows why that leads to a failure to correctly shape-simulate $\calT$.

\begin{enumerate}
    \item Location of $A$: Since there exist terminal assemblies of $\calT$ which have green tiles north of $A$ capped by a red tile, and also tiles to the east of $A$, with no connected path between them other than through $A$, it must be the case that tiles can attach in $\mathcal{S}$ to both the north and the east of the tile of $\sigma'$.  Let $n = |S|$ be the number of tile types in $\mathcal{S}$, and note that in $\calT$ there exist terminal assemblies where the green columns of tiles grow to a height of $h > n$. In order for $\calS$ to shape-simulate $\calT$, it must also be able to grow columns of tiles in the locations of green tiles to a height of $> h$. Note that this means that some tile type of $S$ must appear in such a column more than once, and since it is only a single-tile-wide column of tiles with a repeating tile type, it must be possible to ``pump'' it up arbitrarily far (i.e. there exists a valid assembly sequence in $\mathcal{S}$ which can grow a column in the location of the green tiles of $\calT$ arbitrarily tall).
    
    Furthermore, since $\mathcal{S}$ is assumed to shape-simulate $\calT$, it must be possible for tiles to grow so that they form a loop similar to that created by the green and blue tiles of $\calT$ (which we'll call a ``north loop'').
    
    First, assume that the ``blue portion'' can grow from the ``green column''. [TODO: show this means there is a valid assembly sequence in which the blue passes the location of $E$, which is invalid.]
    
    [TODO: make images of invalid assemblies from the cases]
    
    Since that cannot be the case, the ``blue portion'' must grow upward from the $E$ location. [TODO: could pump green to a taller height and then crash blue into it, which is invalid.]
    
    \item Locations of $B$, $C$, or $D$: The same argument holds as for the location of $A$. (With the slight caveat of a connected path which avoids $C$ connecting $A$ and $E$, which doesn't change the argument

    \item Location of $E$: Although $E$ is now in place to block the north loop before it begins, an analogous argument that was used for location $A$ can now be used to show that the south loop cannot be correctly grown. [TODO: formalize]
    
    \item Location of a green tile: We can use the same argument as for the location of $A$.
    
    \item Location of a blue tile: [TODO: similar to green]
    
    \item Location of a yellow tile: [TODO: similar to green]
    
    \item Location of a pink tile: [TODO: similar to blue]
\end{enumerate}

The above case analysis shows that there is no location, within the shape of a valid terminal assembly of $\calT$, in which $\sigma'$ can be placed and $\calS$ can then shape-simulate $\calT$. Therefore, $\calS$ does not shape-simulate $\calT$, and since the only assumption made about $\calS$ was that it is singly-seeded, no singly-seeded aTAM system can shape-simulate $\calT$ at scale factor 1.


[TODO: to finish the proof for the full class...]
To add infinitely many additional aTAM systems to $\mathfrak{T}$, we could extend the seed arbitrarily far in either direction and could have arbitrarily more upward and/or downward growing arms/loops along those extensions. It is clear that the previous case analysis could be extended to any such system to show that it also cannot be shape-simulated by any singly-seeded aTAM system.

Therefore, we have shown an infinite class of aTAM systems, $\mathfrak{T}$, such that none can be shape-simulated by any singly-seeded aTAM system at scale factor 1 and thus Theorem~\ref{thm:imposs-scale1} is proven.

\end{proof}


\begin{corollary}\label{cor:imposs-scale1}
There exists an infinite class of aTAM systems, $\mathfrak{T}$, such that for every $\mathcal{T} \in \mathfrak{T}$, there exists no singly-seeded aTAM system $\mathcal{S}$ which seed-growth-simulates $\mathcal{T}$ at scale factor 1.
\end{corollary}

\begin{proof}
Corollary \ref{cor:imposs-scale1} follows immediately from Theorem \ref{thm:imposs-scale1} since seed-growth-simulation implies shape-simulation.
\end{proof}


\begin{figure}
    \centering
    \includegraphics[width=0.7\textwidth]{images/scale2-T.png}
    \caption{An example aTAM system $\mathcal{T} = (T,\sigma,1)$ which cannot be shape-simulated at scale factor 2. The grey and green tiles represent the seed tiles (which have unshown strength-1 glues between all adjacent sides). The blue tiles can attach to the green tiles of the seed and nondeterministically allow for growth from any green tile that could potentially crash into the seed at any location.}
    \label{fig:scale2-T}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{images/no-single-seed-at-scale-factor-2.png}
    \caption{The system shown in Figure~\ref{fig:scale2-T} at scale factor 2. Each $2 \times 2$ block represents one tile of the seed of $\calT$. Green blocks represent locations from which growth can be initiated outward from the seed.}
    \label{fig:no-single-seed-at-scale-factor-2}
\end{figure}


\begin{theorem}\label{thm:imposs-scale2}
There exists an infinite class of aTAM systems, $\mathfrak{T}$, such that for every $\mathcal{T} \in \mathfrak{T}$, there exists no singly-seeded aTAM system $\mathcal{S}$ which shape-simulates $\mathcal{T}$ at scale factor $\le 2$.
\end{theorem}

\begin{proof}
For the proof of Theorem \ref{thm:imposs-scale2}, we present an aTAM system $\mathcal{T} = (T,\sigma,1)$ and show that no singly-seeded aTAM system can shape-simulate it at scale factor $\le 2$. Figure \ref{fig:scale2-T} shows $\mathcal{T}$ and Figure \ref{fig:no-single-seed-at-scale-factor-2} depicts a version at scale factor 2.

Our proof will be by contradiction, so assume that there exists an aTAM system $\mathcal{S} = (S,\sigma_\mathcal{S},\tau)$ which shape-simulates $\calT$ at scale factor 2.

We first note that the green tiles of the seed of $\calT$ allow for the attachment of blue tiles. From each green tile, it is possible for a path of blue tiles to attach which can (1) be arbitrarily long, and (2) grow to any location on the perimeter of the seed. The nondeterministic nature of the aTAM means that any such path has a possibility of growing from any one green tile before a single tile attaches to any other green lite. We will only focus on such paths which grow far enough away from the seed then turn and grow a straight line path into a location adjacent to the seed such that the path that returns to the seed ``pumps'' (TODO: refer to the Window Movie Lemma). We will call such a path a ``crashing path'' .

Since every green location can initiate growth of a crashing path which can crash into any other green location, and since such a crashing path must be able to resolve a tile of a blue type in a location where a green tile should be if there is no tile already in the green macrotile location, it must be the case that before any crashing path can grow, at least one tile is present in each green macrotile location. [TODO: there are a few trivial details to walk through to make this completely clear.]

Since $\mathcal{S}$ is singly-seeded, $\sigma_\mathcal{S}$ can have at most a single tile in a single green macrotile location. Without loss of generality, assume that $\sigma_\mathcal{S}$ consists of a tile in the green macrotile location $A$. (If not, it must grow a path to a green macrotile location, w.l.o.g. assume $A$ is the first, and our argument continues from that point.) It must be the case that a non-branching path grows from $A$ to every other green macrotile location before any of them can initiate growth of a simulated crashing path (by our previous argument). We will call this path the ``blocking path'' and without loss of generality assume that the first green macrotile to have a tile is $A$ and the last is $E$. (Our arguments will apply for any other choices.)

Because it must not be possible to initiate growth of any crashing path before completion of the blocking path, i.e. the blocking path must first place at least $1$ tile in each green macrotile, after the blocking path places a tile in the last green macrotile location it must then initiate growth of paths that go to every other green macrotile location to allow them to initiate growth of crashing paths. We call these paths ``activation paths''.

We now analyze the paths that must grow. It $A$ is the first and $E$ the last macrotile on the path, then $B$ and $D$ must be visited in between. Since the path cannot branch, it must be the case that it grows upward to, then back down from, each of $B$ and $D$. This requires the use of two tile locations across the cuts marked as diagonal red lines. (The outlined locations show all valid locations for tile placements allowed strictly during growth of the seed, accounting for allowable fuzz. The missing $2\times 2$ square would be the location of invalid diagonal fuzz.) Once the blocking path completes at $E$, it must then be the case that activation paths grow back to both $B$ and $D$, using the third of the four valid tile locations along the red cuts. However, at least one of either the path to $B$ or $D$ must then continue to activate $C$. (This is because the blocking path will have cut $C$ off from any paths except those that go around the blocking path at those locations.) In order to do this, that path would require use of the fourth of four locations along the associate red diagonal. At this point, one of the macrotile locations marked as yellow must be completely filled. By the definition of simulation, since no additional tiles can ever be added to that macrotile, whatever tile in $\calT$ that it maps to at this point must be permanent. If it now maps to a tile (rather than empty space), we can grow crashing paths that miss that location, yielding an invalid assembly. If it maps to empty space, we can instead grow a crashing path that should terminate in that location but is unable to do so, also yielding an invalid assembly.

[TODO: more details are needed. I'm trying to prove the stronger statement of shape self-assembly and need to make sure that there isn't some weird nondeterministic crap that could occur. I don't think so because of pumping...]

%Furthermore, after placing the first tile in any green macrotile other than the final visited by the path, that macrotile cannot yet be able to grow a crashing path (by our previous argument) and therefore after visiting the final green macrotile the path must return to each other to place at least one more tile, allowing each to begin possible growth of crashing paths. Note that the return path need no longer be a single, un-branching path, though.

%Without loss of generality, assume that green macrotile $A$ receives the first tile. There must be a path from $A$ to each other green macrotile. 


% Proof sketch:
% \begin{enumerate}
%     \item Without loss of generality
%     \item 2 paths needed to block
%     \item 1 needed to activate
%     \item 1 to continue back
%     \item There is a cut of size 4
%     \item Therefore would have to fill a fuzz location(!?)
%     \item If something could crash into that fuzz location later: FAIL
%     \item There must be a path between C and F before activation
%     \item In order to activate C, a path must travel from either B or D
%     \item Therefore, X or Z must remain open until the path to C grows
%     \item That can only happen if the fuzz in the yellow locations becomes filled
% \end{enumerate}

\end{proof}




==> imposs-scale3.tex <==
\section{Seed-Growth-Simulation at Scale Factor 3}

\begin{theorem}\label{thm:imposs-scale3}
There exists an infinite set of poly-seeded aTAM systems such that none of them can be seed-growth simulated by any singly-seeded aTAM system at scale factor $\le 3$ without the use of cheating fuzz.
\end{theorem}

[TODO: the proof of Theorem \ref{thm:imposs-scale2} applies directly to this, so the following proof should be removable.]

Throughout the following, a \emph{single-tile-wide path} of tiles in an assembly $\alpha$ is an ordered sequence of tiles $(t_0,t_1,...,t_{n-1})$ such that, for $0<i<n$, $t_i$ binds to $\alpha$ via a single $\tau$-strength glue on $t_{i-1}$.

The following lemma states that if arbitrarily long paths can grow and crash into tiles of a system's seed, then any system which seed-growth-simulates that system must ensure that all those locations which map (under the representation function) to those seed locations which can be crashed into must have tiles within them before those crashing paths can grow.

\begin{lemma}\label{lem:seed-first}(Seed First Lemma)
Let $\calT = (T,\sigma_\calT,\tau)$ be a poly-seeded aTAM system, and let $\mathcal{S}$ be a singly-seeded aTAM system which seed-growth-simulates $\calT$. Let $L \subseteq \dom \sigma_\calT$ be a set of locations in the seed of $\calT$ such that for any value $d \in \mathbb{Z}^+$, for each $l \in L$, there exists a valid assembly sequence in $\calT$ where a single-tile-wide path of tiles, $p_l$, begins at distance $d$ away from $l$ and grows until the tile at location $l$ blocks further growth of $p_l$. For each $l$, let $C_l$ be the set of all such unique paths $p_l$ which can crash into $l$ (across all valid assembly sequences) such that, if the seed tile was not in location $l$, a tile of a different type would be able to attach in location $l$ by attaching to the last tile placed in $p_l$. In $\calS$, for each $l \in L$ the macrotile location which maps to location $l$ must have at least one tile within it before it is possible to grow the path of macrotiles which represent any $p_l \in C_l$.
\end{lemma}

\begin{proof}
We prove Lemma~\ref{lem:seed-first} by contradiction. Therefore, assume that in $\calS$ there exists a macrotile which maps to a location $l \in L$ which has no tiles in it, and macrotiles which represent some $p_l \in C_l$ are able to assemble. %Let $c$ be the scale factor by which $\calS$ simulates $\calT$.

First, we note that by the Window Movie Lemma of \cite{temp1notIU}, that there is a constant $p$ such that, if $p_l$ grows beyond length $p$ (which must be possible by the definition of the paths in $C_l$), there must be valid assembly sequences which allow $p_l$ to become ``pumpable''. That is, there must exist at least two separate cuts in the binding graph across the macrotiles representing $p_l$ with identical window movies (i.e. the same glues attaching in the same order), which means there is a valid assembly sequence allowing the assembly between those cuts to be repeated arbitrarily many times (i.e. pumped) unless growth collides with previously existing tiles. Therefore, $p_l$ must be able to grow a macrotile which represents the next tile of $p_l$ into the empty seed tile location. This would be a failure of $\mathcal{s}$ to correctly (seed-growth-)simulate $\calT$. Therefore, every such $l \in L$ must have at least one tile within in to prevent that growth.
\end{proof}

\begin{definition}
A \emph{precedence path} in an assembly $\alpha$ is a path in the biding graph of $\alpha$ following an ordered sequence of tiles in $\alpha$, $(t_0,t_1,...t_{n-1})$, such that for each $0<i<n$, tile $t_{i-1}$ provides an output glue which is necessary for the biding of an input glue on $t_i$ to allow it to bind into $\alpha$. 
\end{definition}

[TODO: rework the following lemma by defining locations that ``output'' (i.e. allow the growth away from the seed which eventually crashes) and then saying that no location can output until all locations into which its output can crash must have a precedence path connecting them before the output location grows.]

\begin{lemma}\label{lem:single-path}(Single Path Lemma)
Given the same systems $\calT$ and $\calS$ and sets $L$ and $C_l$ as defined for Lemma~\ref{lem:seed-first}, for every producible assembly in $\calS$ in which macrotiles exist that represent any path $p_l$ in any $C_l$, there exists a precedence path which begins at the seed tile, includes a minimum of one tile in every macrotile representing a location in $L$, and ends with the macrotiles of $p_l$.
\end{lemma}

\begin{proof}
We prove Lemma~\ref{lem:single-path} by contradiction. Therefore, assume that there exists some producible assembly $\beta \in \prodasm{\calS}$ such that $\beta$ contains the macrotiles of some $p_l$ but no precedence path leading from the seed tile to the macrotiles of $p_l$ contains at least one tile in every macrotile representing a location in $L$.
\end{proof}


\begin{proof}
We prove Theorem~\ref{thm:imposs-scale3} by giving a concrete example of a poly-seeded aTAM system $\mathcal{T}$ which cannot be simulated by any singly-seeded aTAM system at scale factor $3$ without the use of cheating fuzz. We will then show how an infinite set of poly-seeded aTAM systems can be derived from that example.

\begin{figure}
    \centering
    \includegraphics[width=1.0\textwidth]{images/no-single-seed-at-scale-factor-3-examples.png}
    \caption{This system should work for a proof that singly-seeding can't work at scale factor 3 without cheating fuzz.[TODO: note that without cheating fuzz, only depicted macrotiles can ever have tiles within them.]}
    \label{fig:no-single-seed-at-scale-factor-3}
\end{figure}

Let $\calT = (T,\sigma,1)$ be the system represented in Figure~\ref{fig:no-single-seed-at-scale-factor-3}, which shows examples of its growth. Note that, in the figure, each tile of $\calT$ is represented as a $3 \times 3$ block of squares surrounded by a darker line, thus showing the subdivision of the macrotiles of a simulator at scale 3 which is attempting to simulate $\calT$. The grey blocks represent locations within the seed $\sigma$.

The tiles at the locations labeled $X$ and $Y$ both initiate growth of northward and southward columns which nondeterministically grow to arbitrary lengths before either randomly being ``capped' by a red tile or growing right, or left (respectively) one of two fixed distances before then growing columns which eventually crash back into the seed locations $A$,$B$,$C$, or $D$.

The intuitive reason behind why $\calT$ cannot be seed-growth-simulated by a singly-seeded system is that, in $\calT$, all 4 locations $A$,$B$,$C$, and $D$ of the seed are tiled before any non-seed growth can occur, and therefore they are in place and able to block any growth which might eventually crash into them. Assume, for the sake of contradiction, that some singly-seeded aTAM system $\mathcal{S}$ seed-growth-simulates $\calT$. [TODO: switch to reference the Seed First Lemma]

If there is a valid assembly sequence in $\mathcal{S}$ in which such a column grows through one of the locations $A$,$B$,$C$, or $D$, then $\mathcal{S}$ fails to (seed-growth-)simulate $\calT$. Therefore, it must be the case that before any such column can validly grow, starting from $X$ or $Y$, there exists at least one tile in each macrotile location corresponding to $A$,$B$,$C$, and $D$. However, since $\mathcal{S}$ is singly-seeded, at most one location in one of the grey macrotiles can have $\mathcal{S}$'s seed tile, and then one or more paths of tiles must grow which place tiles so that there is at least one tile in each of the macrotiles in locations $A$,$B$,$C$, and $D$.

We first show that it must be a single, unbranching path which grows into each of the macrotiles representing locations $A$,$B$,$C$, and $D$ and only after doing so can growth of the macrotiles at $X$ and $Y$ complete to the point that they can grow upward or downward columns (which we will refer to as ``outputting''). Therefore, assume otherwise, namely that growth of a path $p_{xy}$ can occur into at least one of the macrotiles of $X$ or $Y$ and allow it to output, and that $p_{xy}$ is independent of (i.e. a separate path or a branch off of) any path which places a tile in at least one of $A$,$B$,$C$, or $D$. (Without loss of generality, we will assume that $p_{xy}$ grows into $X$, and that $p_{xy}$ is independent of any path growing into $A$.) This means that there exists a valid assembly sequence in $\mathcal{S}$ in which $p_{xy}$ grows into $X$, then a column grows upward out of $X$ to length $\ge l$, then growth representing blue tiles occurs which grows rightward to a location over $A$, and then a column grows downward. If $\mathcal{S}$ correctly simulates $\calT$, that downward growing column must be able to grow to length $>l$. [TODO: make use of the Seed First Lemma]

Thus, by the following argument, it must be the case that a single, unbranching path (which we'll call $p$) grows from the single seed tile of $\mathcal{S}$, places at least one tile in each of $A$,$B$,$C$, and $D$, and only then can growth continue (now via one or more paths) into locations $X$ and $Y$ and allow them to output.

\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{images/no-single-seed-at-scale-factor-3-pathss.png}
    \caption{Possible paths through the macrotiles of $\mathcal{S}$ which represent the seed of $\calT$.}
    \label{fig:no-single-seed-at-scale-factor-3-paths}
\end{figure}

Without loss of generality, assume that either (1) the seed tile of $\mathcal{S}$ is in the macrotile of $A$, or (2) path $p$ visits $A$ before visiting $B$,$C$, or $D$. Figure~\ref{fig:no-single-seed-at-scale-factor-3-paths} shows possible routes for $p$. The left two show possible routes if $B$ is visited before $C$ and $D$, with the differences being whether $C$ or $D$ is visited next. In the leftmost, $D$ is visited last, so (as previously shown) only from that point can one or more paths grow to $X$ and $Y$ and allow them to output. However, since the macrotiles marked as $C'$ and $B'$ must necessarily each have two rows of tiles across them, it is impossible for any path to grow from $D$ to $X$, thus $X$ can never output and the simulation fails. In the middle image of Figure~\ref{fig:no-single-seed-at-scale-factor-3-paths}, $C$ is visited last by $p$ but then it is impossible to grow a path from there to $Y$, so the simulation would fail. The final case to consider is depicted in the rightmost image of Figure~\ref{fig:no-single-seed-at-scale-factor-3-paths}, in which $C$ and $D$ are visited by $p$ before $B$. However, in this case, depending on which two columns of the macrotiles in the vertical section of the path are occupied, either $X$ or $Y$ cannot be reached by a path. Therefore, in all cases the simulation fails, and therefore $\mathcal{S}$ cannot correctly seed-growth-simulate $\calT$ and there can be no such simulator.

We now show that there is an infinite class of systems of which $\calT$ is a member. It is trivial to build them by making systems similar to $\calT$ but with successively wider seeds, each with its sets of colored tiles modified by adding extra tiles so that the collisions with locations $A$,$B$,$C$, and $D$ can still occur.
 
To prove the final point of Theorem~\ref{thm:imposs-scale3}, that it holds for scale factors 1 and 2 as well, we simply note that no simulator could succeed in growing the necessary paths with even less allowed space than $\mathcal{S}$ was given at scale factor 3.
\end{proof}

% Finally, we demonstrate that an arbitrary aTAM tileset is able to be seed-growth-simulated at scale factor 3, utilizing cheating fuzz.
% The construction of this simulating tileset $\mathcal{T}_3$ consists of three main parts.
% First, we create a tileset $T_\sigma$ which assembles a scale-3 version of seed $\sigma$ in $T$.
% This is the brunt of the construction, and is carried out by an algorithm which utilizes the fact that all shapes with scale factor $\geq 2$ contain a Hamiltonian cycle to generate a precedence path that allows for all tiles in the seed to be resolved before allowing growth of the remaining assembly.
% We call the precedence path which represents the Hamiltonian cycle the \emph{core path} (TODO: maybe change?).
% The south-westernmost tile is selected as the \emph{origin} tile, and we select the macrotile used to represent it (see Figure~\ref{fig:S3-8_origin_macrotile}) in $T_\sigma$ by its neighbors.
% As a result of the selection of the origin macrotile, a new single-tile seed $\sigma_0$ can then provided.
% A set of macrotiles (see Figure~\ref{fig:S3-2_seed_path_macrotiles}) are used as templates for each tile, and are assigned by the creation of a depth-first tree from the origin.
% These macrotiles define the core path, as shown by the colored arrows.
% Once the core path is defined we generate a second precedence path, the \emph{external path} (TODO: this actually isn't a precedence path, as we could potentially have collisions which `cut' the precedence path into smaller segments. A semi-precedence path? Nucleation-restricted path?).

% Second, we create scale-3 versions of the tileset $T$.
% In addition to simply providing new scaled version of the tiles, we additionally need to prevent the re-growth of a seed by glues which may map to macrotiles in the seed.
% Re-growth is prevented by generating a $T_{IO}$ which codes all possible $\tau$ strength combinations which would allow a tile to grow.

% \begin{theorem}\label{thm:scale3-sim}
% Given an arbitrary aTAM system $\mathcal{T} = (T,\sigma,\tau)$, there exists an aTAM system $\mathcal{T}_3$ which seed-growth-simulates $\mathcal{T}$ at scale factor 3, requiring cheating fuzz.
% \end{theorem}

% \begin{proof}
% We prove Theorem~\ref{thm:scale3-sim} by construction.
% Let $\mathcal{T} = (T,\sigma,\tau)$ be an arbitrary aTAM system.  
% We generate the tile system $\mathcal{T}_3 = \left(\{T_3 \cup T_\sigma\}, \sigma_0, \tau_3=2 \right)$ taking as input tileset $T$ and seed $\sigma$.
% The first step is to generate the tileset $T_\sigma$ which allows for growth of the seed assembly.
% We utilize the following steps within an algorithm to create a template for all macrotiles which allows for the creation of tiles which allow for seed-first simulation.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.3\textwidth]{images/S3-8_origin_macrotile.png}
%     \caption{The 3 possible origin macrotiles of westernmost tile of the southernmost row (TODO: some better description?) of the shape. `N/E' is the case where the origin macrotile is connected to two neighbors along both its North and East edges, whereas N and E are connected to only one neighbor along their North or East edge, respectively. Red dots connected to arrows indicate the seed tiles. Green bars indicate location of the final tile of the precedent path. Note that the `N/E' origin contains two precedence paths}
%     \label{fig:S3-8_origin_macrotile}
% \end{figure}

% [TODO: formalize this algorithm]
% \begin{enumerate}
% \item In the initial scale-1 seed $\sigma$, we define the south-westernmost tile of the seed as the \emph{origin} [TODO - potentially tighten this up using min].
% \item 
% \item Create a binding graph of the seed and carry out a depth-first search, where the node in the graph correlating to $\sigma$ is the root of the depth-first spanning tree. For reasons that will be discussed at a later point, the depth first search investigates the `leftmost' neighbor first for `E' growing precedent paths, `rightmost' neighbors for `N' growing precedence paths.
% \item Generate the tiles within the precedent path macrotiles from the list of possible macrotiles (shown in Figure~\ref{fig:S3-2_seed_path_macrotiles}), including rotated variants.
% \item Generate the outermost tiles of the seed (maybe call external perimeter path?).
%     \begin{itemize}
%         \item From the origin macrotile, place the first tile of the perimeter at the end of the precedent path
%         \item Place tiles in a clockwise fashion adjacent to outermost tiles of each precedent path (Note: glues must be able to handle crashes - i.e. when the perimeter path is `interrupted' by the placement of another tile)
%     \end{itemize}
% \item For each enclosed cavity within the seed, generate an internal perimeter path.
% \begin{itemize}
%     \item Among the macrotiles adjacent to a macrotile of the cavity, identify the one which contains tiles with the highest index of the precedent path (i.e., furthest along).
%     Connect the first tile of this internal perimeter path via a strength 2 glue.
%     \item Add tiles in a counter-clockwise fashion, adjacent to the perimeter path.
%     \item As part of this, demonstrate how this is possible for all
% \end{itemize}
% \end{enumerate}

% \begin{figure}
%     \centering
%     \includegraphics[width=\textwidth]{images/S3-2_seed_path_macrotiles.png}
%     \caption{The macrotile types which allow for the precedence path to follow the depth-first spanning tree. Note, we can rotated these to allow for all possible paths}
%     \label{fig:S3-2_seed_path_macrotiles}
% \end{figure}

% We note that this process is very similar for scale 4, changing out the macrotiles utilized

% For the remaining simulations of $3 \times 3$ tiles, we define the point of cooperativity as the central tile in a $3 \times 3$ square, as shown in Figure~\ref{fig:S3-7_cooperativity_scale3}.
% \end{proof}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.4\textwidth]{images/S3-7_cooperativity_scale3.png}
%     \caption{For a scale 3 macrotile, the point of cooperativity resides in the center of the $3 \times 3$ square (denoted with `C').}
%     \label{fig:S3-7_cooperativity_scale3}
% \end{figure}
